Forbidden Induced Subgraphs for Bounded Shrub-Depth and the Expressive Power of MSO

The graph parameter shrub-depth is a dense analog of tree-depth. We characterize classes of bounded shrub-depth by forbidden induced subgraphs. The obstructions are well-controlled flips of large half-graphs and of disjoint unions of many long paths. Applying this characterization, we show that on every hereditary class of unbounded shrub-depth, MSO is more expressive than FO. This confirms a conjecture of [Gajarsk\'y and Hlin\v{e}n\'y; LMCS 2015] who proved that on classes of bounded shrub-depth FO and MSO have the same expressive power. Combined, the two results fully characterize the hereditary classes on which FO and MSO coincide, answering an open question by [Elberfeld, Grohe, and Tantau; LICS 2012]. Our work is inspired by the notion of stability from model theory. A graph class C is MSO-stable, if no MSO-formula can define arbitrarily long linear orders in graphs from C. We show that a hereditary graph class is MSO-stable if and only if it has bounded shrub-depth. As a key ingredient, we prove that every hereditary class of unbounded shrub-depth FO-interprets the class of all paths. This improves upon a result of [Ossona de Mendez, Pilipczuk, and Siebertz; Eur. J. Comb. 2025] who showed the same statement for FO-transductions instead of FO-interpretations.

==> imports.tex <==
\usepackage{amsthm}
\usepackage{amsmath}
\usepackage{wrapfig}
\usepackage{thm-restate}
\usepackage[font=small]{caption}%make figure captions a bit smaller
% \RequirePackage[osf,sc]{mathpazo}
\usepackage[hidelinks]{hyperref}
\usepackage[capitalise]{cleveref}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage[textsize=tiny]{todonotes}
\usepackage[inline]{enumitem}
\usepackage{mathtools}
\usepackage{cases}
\usepackage[only,llbracket,rrbracket]{stmaryrd}
\newcommand{\smallblacksquare}{{\vcenter{\hbox{\rule{.6ex}{.6ex}}}}}
\usepackage{array}
\usepackage{multirow}
\usepackage{multicol}
\usepackage{mathrsfs} 
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{conjecture}[theorem]{Conjecture}
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{observation}[theorem]{Observation}
\newtheorem{ass}[theorem]{Assertion}
\newtheorem{example}[theorem]{Example}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{property}[theorem]{Property}
\newtheorem{fact}[theorem]{Fact}

\usepackage{enumitem}
\setlist[itemize]{topsep=4pt,itemsep=3pt,parsep=0pt} 
\setlist[enumerate]{topsep=4pt,itemsep=3pt,parsep=0pt} 

% \usepackage{lineno}
% \linenumbers


\Crefname{figure}{Figure}{Figures}

\renewcommand{\cal}{\mathcal}



\renewcommand{\preceq}{\preccurlyeq}
\renewcommand{\int}{\mathrm{int}}
\newcommand{\const}{\mathrm{const}}

\newcommand{\rk}{\mathrm{rk}}
\newcommand{\rw}{\mathrm{rankwidth}}
\newcommand{\cw}{\mathrm{cliquewidth}}

\newcommand{\bu}{\bar u}
\newcommand{\bv}{\bar v}
\newcommand{\bw}{\bar w}
\newcommand{\bx}{\bar x}
\newcommand{\by}{\bar y}
\newcommand{\bz}{\bar z}

\newcommand{\wh}{\widehat}
\newcommand{\conv}{\mathrm{Conv}}

\newcommand{\NN}[0]{\mathrm{\mathbb{N}}}
\newcommand{\N}[0]{\mathrm{\mathbb{N}}}

\newcommand{\tp}{\mathrm{tp}}
\newcommand{\otp}{\mathrm{otp}}
\newcommand{\etp}{\mathrm{etp}}
\newcommand{\atp}{\mathrm{atp}}
\newcommand{\ex}{\mathrm{ex}}
\renewcommand{\subset}{\subseteq}
\newcommand{\row}{\textnormal{row}}
\newcommand{\col}{\textnormal{col}}
\newcommand{\column}{\textnormal{column}}
\newcommand{\dist}{\textnormal{dist}}
\newcommand{\type}{\textnormal{type}}
\newcommand{\qtype}{\tp_q}
\newcommand{\suff}{\textnormal{suff}}
\newcommand{\pref}{\textnormal{pref}}
\renewcommand{\phi}{\varphi}
\newcommand{\card}{\mathrm{card}}
\newcommand{\plusplus}{%
  \mathbin{{+}\mspace{-8mu}{+}}%
}
\newcommand{\XOR}{\textnormal{~~XOR~~}}

\newcommand{\Start}{\mathrm{start}}
\newcommand{\End}{\mathrm{end}}

\newcommand{\LL}{\mathcal{L}}
\newcommand{\lc}{\mathrm{lc}}
\newcommand{\str}[1]{\mathbb{#1}}
\newcommand{\flip}{\mathrm{flip}}
\newcommand{\prep}{\mathrm{prep}}
\newcommand{\T}{\mathrm{reserved}}
\newcommand{\DD}{\mathcal{D}}
\newcommand{\BB}{\mathcal{B}}
\newcommand{\TT}{\mathcal{T}}
\newcommand{\II}{\mathcal{I}}
\newcommand{\XX}{\mathcal{X}}

\newcommand{\FO}{\mathrm{FO}}
\newcommand{\MSO}{\mathrm{MSO}}
\newcommand{\CMSO}{\mathrm{CMSO}}
\newcommand{\CMSOD}[2]{\mathrm{C}_{#1}\mathrm{MSO}^{(#2)}}

\newcommand{\Bs}{\BB^\star}
\newcommand{\Bc}{\BB^\bullet}
\newcommand{\Bo}{\BB^{\scriptscriptstyle \blacktriangleleft}}
\newcommand{\Bg}{\BB^{\smallblacksquare}}
\newcommand{\twins}{\mathrm{twins}}
\newcommand{\counttwins}{\mathrm{\#twins}}
\newcommand{\flipped}{\mathrm{flipped}}
\newcommand{\dropbounds}[1]{\llbracket#1\rrbracket}

\newcommand{\BBsr}{\overline{\BB^\star_r}}
\newcommand{\BBcr}{\overline{\BB^\bullet_r}}
\newcommand{\BBor}{\overline{\BB^{\scriptscriptstyle \blacktriangleleft}_r}}
\newcommand{\DDD}{\overline{\DD}}


\newcommand{\jan}[1]{\todo[color=orange!40]{Jan: #1}}
\newcommand{\janin}[1]{\todo[inline,size=\normalsize,color=orange!40,caption={}]{Jan: #1}}
\newcommand{\niko}[1]{\todo[color=green!40]{Niko: #1}}
\newcommand{\nikoin}[1]{\todo[inline,size=\normalsize,color=green!40,caption={}]{Niko: #1}}
\newcommand{\szym}[1]{\todo[color=blue!40]{Szymon: #1}}
\newcommand{\szymin}[1]{\todo[inline,size=\normalsize,color=blue!40,caption={}]{Szymon: #1}}
\newcommand{\set}[1]{\{#1\}}
\newcommand{\setof}[2]{\{#1\mid#2\}}
\newcommand{\chn}[3]{\langle #1]_{#2}^{#3}}


\newcommand{\struc}[1]{\mathfrak{#1}}
\newcommand{\gc}[1]{\mathcal{#1}}

\newcommand{\sless}{{\scriptscriptstyle <}}
\newcommand{\sgreater}{{\scriptscriptstyle >}}
\newcommand{\CC}{\mathcal{C}}
\newcommand{\EE}{\mathcal{E}}
\newcommand{\FF}{\mathcal{F}}
\newcommand{\PP}{\mathcal{P}}
\newcommand{\QQ}{\mathcal{Q}}
\newcommand{\RR}{\mathcal{R}}
\renewcommand{\SS}{\mathcal{S}}

\renewcommand{\le}{\leqslant}
\renewcommand{\leq}{\le}
\renewcommand{\ge}{\geqslant}
\renewcommand{\geq}{\ge}
\newcommand{\KK}{\mathcal{K}}
\newcommand{\from}{\colon}

\newenvironment{claimproof}[1][\proofname]{%
  \renewcommand{\qedsymbol}{$\blacksquare$}%
  \begin{proof}[#1]%
}{%
  \end{proof}%
}
\usetikzlibrary{arrows.meta}
